Goldstone Inflation

Identifying the inflaton with a pseudo-Goldstone boson explains the flatness of its potential. Successful Goldstone Inflation should also be robust against UV corrections, such as from quantum gravity: in the language of the effective field theory this implies that all scales are sub-Planckian. In this paper we present scenarios which realise both requirements by examining the structure of Goldstone potentials arising from Coleman-Weinberg contributions. We focus on single-field models, for which we notice that both bosonic and fermionic contributions are required and that spinorial fermion representations can generate the right potential shape. We then evaluate the constraints on non-Gaussianity from higher-derivative interactions, finding that axiomatic constraints on Goldstone boson scattering prevail over the current CMB measurements. The fit to CMB data can be connected to the UV completions for Goldstone Inflation, finding relations in the spectrum of new resonances. Finally, we show how hybrid inflation can be realised in the same context, where both the inflaton and the waterfall fields share a common origin as Goldstones.

==> refs.tex <==
@ARTICLE{
AUTHOR = "A.~H.~Guth",
 TITLE =  "The Inflationary Universe: A Possible Solution to the Horizon and Flatness Problems"
  Phys.\ Rev.\ D {\bf 23}, 347 (1981).
  %%CITATION = PHRVA,D23,347;%%
  }
  
\bibitem{here} 
 K.~Freese, J.~A.~Frieman and A.~V.~Olinto,
  ``Natural inflation with pseudo - Nambu-Goldstone bosons,''
  Phys.\ Rev.\ Lett.\  {\bf 65}, 3233 (1990).
  %%CITATION = PRLTA,65,3233;%%
 F.~C.~Adams, J.~R.~Bond, K.~Freese, J.~A.~Frieman and A.~V.~Olinto,
  ``Natural inflation: Particle physics models, power law spectra for large scale structure, and constraints from COBE,''
  Phys.\ Rev.\ D {\bf 47}, 426 (1993)
  [hep-ph/9207245].
  %%CITATION = HEP-PH/9207245;%%
  
\bibitem{wmap}
E.~Komatsu {\it et al.}  [WMAP Collaboration],
  ``Seven-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Interpretation,''
  Astrophys.\ J.\ Suppl.\  {\bf 192}, 18 (2011)
  [arXiv:1001.4538 [astro-ph.CO]].
  %%CITATION = ARXIV:1001.4538;%%

\bibitem{Planck} 
 P.~A.~R.~Ade {\it et al.}  [Planck Collaboration],
  ``Planck 2013 results. XVI. Cosmological parameters,''
  Astron.\ Astrophys.\  {\bf 571}, A16 (2014)
  [arXiv:1303.5076 [astro-ph.CO]].
  %%CITATION = ARXIV:1303.5076;%%

\bibitem{wormholes}
  R.~Kallosh, A.~D.~Linde, S.~Prokushkin and M.~Shmakova,
  ``Gauged supergravities, de Sitter space and cosmology,''
  Phys.\ Rev.\ D {\bf 65} (2002) 105016
  [hep-th/0110089].
  %%CITATION = HEP-TH/0110089;%%

\bibitem{hybrid} 
A.~D.~Linde,
  ``Hybrid inflation,''
  Phys.\ Rev.\ D {\bf 49}, 748 (1994)
  [astro-ph/9307002].
  %%CITATION = ASTRO-PH/9307002;%%
  
  \bibitem{Peloso} 
  J.~E.~Kim, H.~P.~Nilles and M.~Peloso,
  ``Completing natural inflation,''
  JCAP {\bf 0501}, 005 (2005)
  [hep-ph/0409138].

\bibitem{N-flation}
 S.~Dimopoulos, S.~Kachru, J.~McGreevy and J.~G.~Wacker,
 ``N-flation,''
  JCAP {\bf 0808} (2008) 003
  [hep-th/0507205].
  %%CITATION = HEP-TH/0507205;%%

\bibitem{axion-monodromy}
 E.~Silverstein and A.~Westphal,
  ``Monodromy in the CMB: Gravity Waves and String Inflation,''
  Phys.\ Rev.\ D {\bf 78}, 106003 (2008)
  [arXiv:0803.3085 [hep-th]].
  %%CITATION = ARXIV:0803.3085;%%

 \bibitem{pseudonat}
 N.~Arkani-Hamed, H.~C.~Cheng, P.~Creminelli and L.~Randall,
  ``Pseudonatural inflation,''
  JCAP {\bf 0307}, 003 (2003)
  [hep-th/0302034].
  %%CITATION = HEP-TH/0302034;%% 
  
\bibitem{extra-natural} 
 N.~Arkani-Hamed, H.~C.~Cheng, P.~Creminelli and L.~Randall,
  ``Extra natural inflation,''
  Phys.\ Rev.\ Lett.\  {\bf 90}, 221302 (2003)
  [hep-th/0301218].
  %%CITATION = HEP-TH/0301218;%%

\bibitem{extranat2}
 K.~Kohri, C.~S.~Lim and C.~M.~Lin,
  ``Distinguishing between Extra Natural Inflation and Natural Inflation after BICEP2,''
  JCAP {\bf 1408} (2014) 001
  [arXiv:1405.0772 [hep-ph]].
  %%CITATION = ARXIV:1405.0772;%%
  
  \bibitem{multinatural}
  M.~Czerny and F.~Takahashi, ``Multi-Natural Inflation,''  
Phys.\ Lett.\ B {\bf 733}, 241 (2014) [arXiv:1401.5212 [hep-ph]]

\bibitem{LH} 
 N.~Arkani-Hamed, A.~G.~Cohen, E.~Katz, A.~E.~Nelson, T.~Gregoire and J.~G.~Wacker,
  ``The Minimal moose for a little Higgs,''
  JHEP {\bf 0208}, 021 (2002)
  [hep-ph/0206020].
  %%CITATION = HEP-PH/0206020;%%
  
\bibitem{Composite-Higgs-orig} 
R.~Contino, Y.~Nomura and A.~Pomarol,
  ``Higgs as a holographic pseudoGoldstone boson,''
  Nucl.\ Phys.\ B {\bf 671} (2003) 148
  [hep-ph/0306259].
  %%CITATION = HEP-PH/0306259;%%
  
\bibitem{John}
 C.~Csaki, N.~Kaloper, J.~Serra and J.~Terning,
  ``Inflation from Broken Scale Invariance,''
  Phys.\ Rev.\ Lett.\  {\bf 113}, 161302 (2014)
  [arXiv:1406.5192 [hep-th]].
  %%CITATION = ARXIV:1406.5192;%%
  %5 citations counted in INSPIRE as of 27 Nov 2014
    J.~Ellis, N.~E.~Mavromatos and D.~V.~Nanopoulos,
  ``Starobinsky-Like Inflation in Dilaton-Brane Cosmology,''
  Phys.\ Lett.\ B {\bf 732} (2014) 380
  [arXiv:1402.5075 [hep-th]].
  %%CITATION = ARXIV:1402.5075;%%
  %10 citations counted in INSPIRE as of 27 Nov 2014
  
\bibitem{coleman-aspects} 
S.~Coleman,
  ``Aspects of Symmetry: Selected Erice lectures,''
  Cambridge University Press (1985).
 
\bibitem{witten}
P.~Svrcek and E.~Witten,
  ``Axions In String Theory,''
  JHEP {\bf 0606}, 051 (2006)
  [hep-th/0605206].
  %%CITATION = HEP-TH/0605206;%%
  
\bibitem{csaki-terning} 
 C.~Csaki and H.~Murayama,
  ``Instantons in partially broken gauge groups,''
  Nucl.\ Phys.\ B {\bf 532}, 498 (1998)
  [hep-th/9804061].
  %%CITATION = HEP-TH/9804061;%%

\bibitem{Freese-Kinney}
 K.~Freese and W.~H.~Kinney,
  ``Natural Inflation: Consistency with Cosmic Microwave Background Observations of Planck and BICEP2,''
  arXiv:1403.5277 [astro-ph.CO].
  %%CITATION = ARXIV:1403.5277;%%
   K.~Freese, C.~Savage and W.~H.~Kinney,
  ``Natural Inflation: The Status after WMAP 3-year data,''
  Int.\ J.\ Mod.\ Phys.\ D {\bf 16}, 2573 (2008)
  [arXiv:0802.0227 [hep-ph]].
  %%CITATION = ARXIV:0802.0227;%%
  

\bibitem{xavier} 
 X.~Calmet and V.~Sanz,
  ``Excursion into Quantum Gravity via Inflation,''
  Phys.\ Lett.\ B {\bf 737}, 12 (2014)
  [arXiv:1403.5100 [hep-ph]].
  %%CITATION = ARXIV:1403.5100;%%



\bibitem{burgess}
 C.~P.~Burgess, M.~Cicoli and F.~Quevedo,
  ``String Inflation After Planck 2013,''
  JCAP {\bf 1311}, 003 (2013)
  [arXiv:1306.3512 [hep-th]].
  %%CITATION = ARXIV:1306.3512;%%
  
\bibitem{1410.3808v1} 
 M.~A.~Amin, M.~P.~Hertzberg, D.~I.~Kaiser and J.~Karouby,
  ``Nonperturbative Dynamics Of Reheating After Inflation: A Review,''
  arXiv:1410.3808 [hep-ph].
  %%CITATION = ARXIV:1410.3808;%%
  
\bibitem{1110.3327v1} 
N.~Barnaby, E.~Pajer and M.~Peloso,
  ``Gauge Field Production in Axion Inflation: Consequences for Monodromy, non-Gaussianity in the CMB, and Gravitational Waves at Interferometers,''
  Phys.\ Rev.\ D {\bf 85}, 023525 (2012)
  [arXiv:1110.3327 [astro-ph.CO]].
  %%CITATION = ARXIV:1110.3327;%%
  
\bibitem{0908.4089v2}
 M.~M.~Anber and L.~Sorbo,
  ``Naturally inflating on steep potentials through electromagnetic dissipation,''
  Phys.\ Rev.\ D {\bf 81}, 043534 (2010)
  [arXiv:0908.4089 [hep-th]].
  %%CITATION = ARXIV:0908.4089;%%

\bibitem{japanese_wilson} 
 H.~Hatanaka, T.~Inami and C.~S.~Lim,
  ``The Gauge hierarchy problem and higher dimensional gauge theories,''
  Mod.\ Phys.\ Lett.\ A {\bf 13}, 2601 (1998)
  [hep-th/9805067].
  %%CITATION = HEP-TH/9805067;%%

\bibitem{deconstruction}
 N.~Arkani-Hamed, A.~G.~Cohen and H.~Georgi,
  ``(De)constructing dimensions,''
  Phys.\ Rev.\ Lett.\  {\bf 86}, 4757 (2001)
  [hep-th/0104005].
  %%CITATION = HEP-TH/0104005;%%
  %596 citations counted in INSPIRE as of 24 Nov 2014
  C.~T.~Hill, S.~Pokorski and J.~Wang,
  ``Gauge invariant effective Lagrangian for Kaluza-Klein modes,''
  Phys.\ Rev.\ D {\bf 64}, 105005 (2001)
  [hep-th/0104035].
  %%CITATION = HEP-TH/0104035;%%

\bibitem{deconstr-EWSB}
  N.~Arkani-Hamed, A.~G.~Cohen and H.~Georgi,
  ``Electroweak symmetry breaking from dimensional deconstruction,''
  Phys.\ Lett.\ B {\bf 513}, 232 (2001)
  [hep-ph/0105239].
  %%CITATION = HEP-PH/0105239;%%
  
\bibitem{adscft}
O.~Aharony, S.~S.~Gubser, J.~M.~Maldacena, H.~Ooguri and Y.~Oz,
  ``Large N field theories, string theory and gravity,''
  Phys.\ Rept.\  {\bf 323}, 183 (2000)
  [hep-th/9905111].
  %%CITATION = HEP-TH/9905111;%%

\bibitem{me-interp-others} 
  J.~Hirn and V.~Sanz,
  ``Interpolating between low and high energy QCD via a 5-D Yang-Mills model,''
  JHEP {\bf 0512}, 030 (2005)
  [hep-ph/0507049],
  %%CITATION = HEP-PH/0507049;%%
  ``A Negative S parameter from holographic technicolor,''
  Phys.\ Rev.\ Lett.\  {\bf 97}, 121803 (2006)
  [hep-ph/0606086].
  %%CITATION = HEP-PH/0606086;%%
   ``The Fifth dimension as an analogue computer for strong interactions at the LHC,''
  JHEP {\bf 0703}, 100 (2007)
  [hep-ph/0612239].
  %%CITATION = HEP-PH/0612239;%%

\bibitem{CHM-reviews}
R.~Contino,
  ``The Higgs as a Composite Nambu-Goldstone Boson,''
  arXiv:1005.4269 [hep-ph].
  %%CITATION = ARXIV:1005.4269;%%
   B.~Bellazzini, C.~Csaki and J.~Serra,
  ``Composite Higgses,''
  Eur.\ Phys.\ J.\ C {\bf 74}, 2766 (2014)
  [arXiv:1401.2457 [hep-ph]].
  %%CITATION = ARXIV:1401.2457;%%

\bibitem{HTC}
 J.~Hirn and V.~Sanz,
  ``The Fifth dimension as an analogue computer for strong interactions at the LHC,''
  JHEP {\bf 0703}, 100 (2007)
  [hep-ph/0612239].
  %%CITATION = HEP-PH/0612239;%%
   J.~Hirn, A.~Martin and V.~Sanz,
  ``Benchmarks for new strong interactions at the LHC,''
  JHEP {\bf 0805}, 084 (2008)
  [arXiv:0712.3783 [hep-ph]].
  %%CITATION = ARXIV:0712.3783;%%
    ``Describing viable technicolor scenarios,''
  Phys.\ Rev.\ D {\bf 78}, 075026 (2008)
  [arXiv:0807.2465 [hep-ph]].
  %%CITATION = ARXIV:0807.2465;%%
  
\bibitem{CuredHless}
 G.~Cacciapaglia, C.~Csaki, C.~Grojean and J.~Terning,
  ``Higgsless electroweak symmetry breaking,''
  eConf C {\bf 040802}, FRT004 (2004)
  [Czech.\ J.\ Phys.\  {\bf 55}, B613 (2005)].
  %%CITATION = ECONF,C040802,FRT004;%%
 G.~Cacciapaglia, C.~Csaki, C.~Grojean and J.~Terning,
  ``Curing the Ills of Higgsless models: The S parameter and unitarity,''
  Phys.\ Rev.\ D {\bf 71}, 035015 (2005)
  [hep-ph/0409126].
  %%CITATION = HEP-PH/0409126;%%
   K.~Agashe, C.~Csaki, C.~Grojean and M.~Reece,
  ``The S-parameter in holographic technicolor models,''
  JHEP {\bf 0712}, 003 (2007)
  [arXiv:0704.1821 [hep-ph]].
  %%CITATION = ARXIV:0704.1821;%%
  
\bibitem{ignoble}
 N.~Kaloper, A.~Lawrence and L.~Sorbo,
  ``An Ignoble Approach to Large Field Inflation,''
  JCAP {\bf 1103}, 023 (2011)
  [arXiv:1101.0026 [hep-th]].
  %%CITATION = ARXIV:1101.0026;%%

\bibitem{smolin}
 L.~Smolin,
  ``Gravitational Radiative Corrections as the Origin of Spontaneous Symmetry Breaking!,''
  Phys.\ Lett.\ B {\bf 93}, 95 (1980).
  %%CITATION = PHLTA,B93,95;%%
  
\bibitem{valerie}
 F.~Brummer, V.~Domcke and V.~Sanz,
  ``GUT-scale inflation with sizeable tensor modes,''
  JCAP08 (2014) 066
  [arXiv:1405.4868 [hep-ph]].
  %%CITATION = ARXIV:1405.4868;%%
  
\bibitem{DandVrock} 
  D.~Croon and V.~Sanz,
  %``Saving Natural Inflation,''
  JCAP {\bf 1502}, no. 02, 008 (2015)
  [arXiv:1411.7809 [hep-ph]].
  %%CITATION = ARXIV:1411.7809;%%
  %3 citations counted in INSPIRE as of 24 Mar 2015
  
  %\cite{Ade:2015lrj}
\bibitem{Planck2015} 
  P.~A.~R.~Ade {\it et al.}  [Planck Collaboration],
  %``Planck 2015 results. XX. Constraints on inflation,''
  arXiv:1502.02114 [astro-ph.CO].
  %%CITATION = ARXIV:1502.02114;%%
  %48 citations counted in INSPIRE as of 24 Mar 2015
  
\bibitem{1409.1221} 
  Z.~Kenton and S.~Thomas,
  %``D-brane Potentials in the Warped Resolved Conifold and Natural Inflation,''
  JHEP {\bf 1502}, 127 (2015)
  [arXiv:1409.1221 [hep-th]].
  %%CITATION = ARXIV:1409.1221;%%
  %9 citations counted in INSPIRE as of 24 Mar 2015

\bibitem{transaxions} 
  M.~Montero, A.~M.~Uranga and I.~Valenzuela,
  %``Transplanckian axions !?,''
  arXiv:1503.03886 [hep-th].
  %%CITATION = ARXIV:1503.03886;%%
  %1 citations counted in INSPIRE as of 24 Mar 2015
  
  
  \bibitem{gravityandglobal} 
  R.~Kallosh, A.~D.~Linde, D.~A.~Linde and L.~Susskind,
  %``Gravity and global symmetries,''
  Phys.\ Rev.\ D {\bf 52}, 912 (1995)
  [hep-th/9502069].
  %%CITATION = HEP-TH/9502069;%%
  %183 citations counted in INSPIRE as of 24 mar 2015
  
  %\cite{vonGersdorff:2015fta}
\bibitem{1502.07340} 
  G.~von Gersdorff, E.~Ponton and R.~Rosenfeld,
  %``The Dynamical Composite Higgs,''
  arXiv:1502.07340 [hep-ph].
  %%CITATION = ARXIV:1502.07340;%%
  
  %\cite{Bellazzini:2014yua}
\bibitem{Csakireview} 
  B.~Bellazzini, C.~Csáki and J.~Serra,
  %``Composite Higgses,''
  Eur.\ Phys.\ J.\ C {\bf 74}, no. 5, 2766 (2014)
  [arXiv:1401.2457 [hep-ph]].
  %%CITATION = ARXIV:1401.2457;%%
  %40 citations counted in INSPIRE as of 24 Mar 2015
  
  \bibitem{1102.5343} 
  D.~Baumann and D.~Green,
  %``Equilateral Non-Gaussianity and New Physics on the Horizon,''
  JCAP {\bf 1109}, 014 (2011)
  [arXiv:1102.5343 [hep-th]].
  %%CITATION = ARXIV:1102.5343;%%
  %65 citations counted in INSPIRE as of 24 mar 2015
  
  
  \bibitem{1407.2621} 
  D.~Baumann, D.~Green and R.~A.~Porto,
  %``B-modes and the Nature of Inflation,''
  JCAP {\bf 1501}, no. 01, 016 (2015)
  [arXiv:1407.2621 [hep-th]].
  %%CITATION = ARXIV:1407.2621;%%
  %14 citations counted in INSPIRE as of 24 Mar 2015
  
  
  
%% Jack's additions

\bibitem{Callan69}
C.G.~Callan, S.~Coleman, J.~Wess and B.~Zumino,
``Structure of Phenomenological Lagrangians. II''
Phys. Rev. {\bf177}, 2247 (1969).

\bibitem{Agashe05}
  K.~Agashe, R.~Contino and A.~Pomarol,
  ``The Minimal composite Higgs model,''
  Nucl.\ Phys.\ B {\bf 719}, 165 (2005)
  [hep-ph/0412089].
  %%CITATION = HEP-PH/0412089;%%

\bibitem{Gripaios09}
 B.~Gripaios, A.~Pomarol, F.~Riva and J.~Serra,
  ``Beyond the Minimal Composite Higgs Model,''
  JHEP {\bf 0904}, 070 (2009)
  [arXiv:0902.1483 [hep-ph]].
  %%CITATION = ARXIV:0902.1483;%%

\bibitem{Coleman73}
S.~Coleman and E.~Weinberg,
``Radiative Corrections as the Origin of Spontaneous Symmetry Breaking,''
Phys. Rev. D {\bf 7}, 1888 (1973).

\bibitem{Pomarol12}
A.~Pomarol and F.~Riva,
  ``The Composite Higgs and Light Resonance Connection,''
  JHEP {\bf 1208}, 135 (2012)
  [arXiv:1205.6434 [hep-ph]].
  %%CITATION = ARXIV:1205.6434;%%

\bibitem{tHooft80}
G.~'t Hooft (1980). "Naturalness, Chiral Symmetry and Spontaneous Chiral Symmetry Breaking". In G~'t Hooft,  Recent Developments in Gauge Theories. Plenum Press.

\bibitem{tHooft74}
G.~'t Hooft,
``A planar diagram theory for strong interactions,''
Nucl. Phys. B {\bf72}, 461 (1974); B {\bf75}, 461 (1974).

\bibitem{Witten79}
E.~Witten,
``Baryons in the 1/N expansion'',
Nucl. Phys. B {\bf160}, 57 (1979).

\bibitem{Weinberg67}
S.~Weinberg,
``Precise Relations between the Spectra of Vector and Axial-Vector Mesons,''
Phys. Rev. Lett. {\bf 18} (1967) 507

\bibitem{Knecht97}
M.~Knecht and E.~de Rafael,
  ``Patterns of spontaneous chiral symmetry breaking in the large N(c) limit of QCD - like theories,''
  Phys.\ Lett.\ B {\bf 424}, 335 (1998)
  [hep-ph/9712457].
  %%CITATION = HEP-PH/9712457;%%
